Machine Learning in Precision Medicine to Preserve Privacy via Encryption

Precision medicine is an emerging approach for disease treatment and prevention that delivers personalized care to individual patients by considering their genetic makeups, medical histories, environments, and lifestyles. Despite the rapid advancement of precision medicine and its considerable promise, several underlying technological challenges remain unsolved. One such challenge of great importance is the security and privacy of precision health-related data, such as genomic data and electronic health records, which stifle collaboration and hamper the full potential of machine-learning (ML) algorithms. To preserve data privacy while providing ML solutions, this article makes three contributions. First, we propose a generic machine learning with encryption (MLE) framework, which we used to build an ML model that predicts cancer from one of the most recent comprehensive genomics datasets in the field. Second, our framework's prediction accuracy is slightly higher than that of the most recent studies conducted on the same dataset, yet it maintains the privacy of the patients' genomic data. Third, to facilitate the validation, reproduction, and extension of this work, we provide an open-source repository that contains the design and implementation of the framework, all the ML experiments and code, and the final predictive model deployed to a free cloud service.

==> Preamble-Gloss.tex <==
\usepackage[nopostdot,nonumberlist,numberedsection,section=subsection]{glossaries}
\makenoidxglossaries

\newglossaryentry{breakpoint}
{
  name=breakpoint,
  description={the beginning or end point of a structural variation}
}

\newglossaryentry{copy number}
{
  name=copy number,
  description={number of copies of a particular gene}
}

\newglossaryentry{copy number alteration}
{
  name=copy number alteration,
  description={a change in copy number that has arisen in any cell of the body after conception}
}

\newglossaryentry{chromosome}
{
  name=chromosome,
  description={a molecule that contains part of the \gls{genome} in a condensed, manageable package}
}

\newglossaryentry{chromosomal inversion}
{
  name=chromosomal inversion,
  description={mutation in which a segment of a chromosome is reversed}
}

\newglossaryentry{fusion} { name=fusion, description={when two previously independent genes are
combined or fused together that results from \gls{chromosomal translocation}, \gls{interstitial
deletion}, and \gls{chromosomal inversion}} }

\newglossaryentry{genome}
{
  name=genome,
  description={genetic material of an organism}
}

\newglossaryentry{gene family} { name=gene family, description={a set of several similar genes
formed by duplication, generally with similar function} }

\newglossaryentry{nucleotide}
{
  name=nucleotide,
  description={form the basic structural unit of DNA. Encoded as either A,T,G, or C}
}

\newglossaryentry{HUGO}
{
  name=HUGO,
  description={HUGO(HUman Genome Organization) Gene Nomenclature Committee}
}

\newglossaryentry{HUGO symbol}
{
  name=HUGO symbol,
  description={unique gene identifier derived from the \href{https://www.genenames.org/about/guidelines/}{HUGO gene nomenclature guidelines}}
}

\newglossaryentry{in-frame} { name=in-frame, description={a mutation, where the translation into
protein is not completely disrupted, creating still-functional proteins} }

\newglossaryentry{intergenic}
{
  name=intergenic DNA,
  description={DNA located between genes and are noncoding (i.e. do not encode protein sequences), but occasionally control genes nearby}
}

\newglossaryentry{interstitial deletion} { name=interstitial deletion, description={a mutation in
which part of the DNA (not including the terminal portion of a chromosome) is left out during DNA
replication} }

\newglossaryentry{mutation}
{
  name=mutation,
  description={alteration of the nucleotide sequence of the genome}
}

\newglossaryentry{metastasis}
{
  name=metastasis,
  description={secondary malignant growth distant from the primary site of cancer}
}

\newglossaryentry{mutation signatures}
{
  name=mutation signatures,
  description={characteristic combinations of mutations arising from specific mutation processes}
}

\newglossaryentry{homologous chromosomes}
{
  name=homologous chromosomes,
  description={two chromosomes that carry the same genes, one from each parental source}
}

\newglossaryentry{non-homologous chromosomes}
{
  name=non-homologous chromosomes,
  description={two chromosomes that do not carry the same genes in contrast to \gls{homologous chromosomes}}
}


\newglossaryentry{out-of-frame} { name=out-of-frame, description={a mutation, where the translation
into a protein is completely disrupted, creating non-functional proteins.} }


\newglossaryentry{primary site}
{
  name=primary site,
  description={the location on the body where the first tumor progression begins}
}

\newglossaryentry{somatic}
{
  name=somatic mutation,
  description={genetic alteration acquired by cells that are the progeny of cancerous cells}
}

\newglossaryentry{structural variation}
{
  name=structural variation,
  description={any kind of structural variation to the genome}
}

\newglossaryentry{chromosomal translocation} { name=chromosomal translocation, description={two
types; Robertsonian translocation, which occurs when two \gls{non-homologous chromosomes} get
attached, and reciprocal translocation, which occurs when parts are exchanged between two non-homologous
chromosomes} }


==> preamble-pgfplot.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% general libraries and packages %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{pgf,pgfplots,pgfplotstable,tikz,tkz-fct}
\usepackage{tikz-timing}[2009/12/09]
\usepackage{float,fp}
\usepgflibrary{shapes}
\usepgfplotslibrary{external,statistics}
\usetikzlibrary{calc,trees,positioning,arrows,chains,shapes.geometric,decorations.pathreplacing,decorations.pathmorphing,shapes,matrix,shapes.symbols,er,backgrounds,decorations.text,spy,automata}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% specific settings %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\pgfplotsset{compat=1.11}
\pgfplotsset{width=7cm,compat=1.13}

\newcommand{\NODEUP}{0.5in}
\newcommand{\NODESIDE}{1.2in}
\newcommand{\TRAKSIDE}{2.5in}
\newcommand{\TRAKDOWN}{0.25in}

\newcommand{\MyBoxplotValues}{    [above, font=\tiny]
    node at
    (boxplot whisker cs:\boxplotvalue{lower whisker},1)
    {\pgfmathprintnumber{\boxplotvalue{lower whisker}}}
    node at
    (boxplot box cs: \boxplotvalue{median},1)
    {\pgfmathprintnumber{\boxplotvalue{median}}}
    node at
    (boxplot whisker cs:\boxplotvalue{upper whisker},1)
    {\pgfmathprintnumber{\boxplotvalue{upper whisker}}}
    [below, font=\tiny]
    node at
    (boxplot whisker cs:\boxplotvalue{lower quartile},0)
    {\pgfmathprintnumber{\boxplotvalue{lower quartile}}}
    node at
    (boxplot whisker cs:\boxplotvalue{upper quartile},0)
    {\pgfmathprintnumber{\boxplotvalue{upper quartile}}}
}

\newcommand\INDEX{2} \newcommand\MU{3.2} \newcommand\SIGMA{0.5}

\def\getangle(#1) (#2)#3{%
  \begingroup%
  \pgftransformreset%
  \pgfmathanglebetweenpoints{\pgfpointanchor{#1}{center}}{\pgfpointanchor{#2}{center}}%
  \expandafter\xdef\csname angle#3\endcsname{\pgfmathresult}%
  \endgroup%
}

\tikzset{
  >=stealth',
  punktchain/.style={
    font=\tiny,
    rectangle,
    rounded corners,
    draw=black, very thick,
    text width=7em,
    minimum height=1em,
    text centered},
  line/.style={draw, thick, <-},
  element/.style={
    tape,
    top color=white,
    bottom color=blue!50!black!60!,
    minimum width=8em,
    draw=blue!40!black!90, very thick,
    text width=10em,
    minimum height=1em,
    text centered},
  every join/.style={->, thick,shorten >=1pt},
  decoration={brace},
  tuborg/.style={decorate},
  tubnode/.style={midway, right=2pt},
}


==> sectableweakcorr.tex <==
\begin{tabular}{clllllr}
  \toprule
  $\widehat{S}$ & $\E$ & $\sigma$ & $\RMS(\widehat{S}, S)$ & $\RMS(\widehat{S}, \E S)$ & $\rho_{\widehat{S}, S}$ & $n$\\
  \midrule
  \multicolumn{1}{l}{$S$} & 0.6181 & 0.0434 & 0 & 0.0434 & 1.0000 & \\
  \multicolumn{1}{l}{$\overline{S}$} & 0.8897 & 0.0475 & 0.2774 & 0.2757 & 0.2231 & 20\\
  \multicolumn{1}{l}{$\widehat{S}$} & 0.5914 & 0.0947 & 0.0973 & 0.0984 & 0.2553 & \\\hline

  \multicolumn{1}{l}{$S$} & 0.6231 & 0.0410 & 0 & 0.0410 & 1.0000 & \\
  \multicolumn{1}{l}{$\overline{S}$} & 0.8788 & 0.0499 & 0.2615 & 0.2606 & 0.2991 & 22\\
  \multicolumn{1}{l}{$\widehat{S}$} & 0.5945 & 0.0947 & 0.0956 & 0.0990 & 0.2993 & \\\hline

  \multicolumn{1}{l}{$S$} & 0.6308 & 0.0400 & 0 & 0.0400 & 1.0000 & \\
  \multicolumn{1}{l}{$\overline{S}$} & 0.8656 & 0.0471 & 0.2406 & 0.2395 & 0.2833 & 25\\
  \multicolumn{1}{l}{$\widehat{S}$} & 0.5991 & 0.0865 & 0.0897 & 0.0922 & 0.2946 & \\\hline

  \multicolumn{1}{l}{$S$} & 0.6359 & 0.0358 & 0 & 0.0358 & 1.0000 & \\
  \multicolumn{1}{l}{$\overline{S}$} & 0.8554 & 0.0472 & 0.2253 & 0.2246 & 0.2747 & 28\\
  \multicolumn{1}{l}{$\widehat{S}$} & 0.6035 & 0.0840 & 0.0874 & 0.0901 & 0.2904 & \\\hline

  \multicolumn{1}{l}{$S$} & 0.6469 & 0.0343 & 0 & 0.0343 & 1.0000 & \\
  \multicolumn{1}{l}{$\overline{S}$} & 0.8419 & 0.0439 & 0.2010 & 0.1999 & 0.2434 & 33\\
  \multicolumn{1}{l}{$\widehat{S}$} & 0.6170 & 0.0750 & 0.0792 & 0.0807 & 0.2746 & \\\hline

  \multicolumn{1}{l}{$S$} & 0.6571 & 0.0308 & 0 & 0.0308 & 1.0000 & \\
  \multicolumn{1}{l}{$\overline{S}$} & 0.8246 & 0.0431 & 0.1735 & 0.1730 & 0.2923 & 40\\
  \multicolumn{1}{l}{$\widehat{S}$} & 0.6244 & 0.0711 & 0.0753 & 0.0783 & 0.3185 & \\\hline

  \multicolumn{1}{l}{$S$} & 0.6674 & 0.0271 & 0 & 0.0271 & 1.0000 & \\
  \multicolumn{1}{l}{$\overline{S}$} & 0.8091 & 0.0406 & 0.1473 & 0.1474 & 0.3517 & 50\\
  \multicolumn{1}{l}{$\widehat{S}$} & 0.6357 & 0.0654 & 0.0690 & 0.0727 & 0.3534 & \\\hline

  \multicolumn{1}{l}{$S$} & 0.6808 & 0.0217 & 0 & 0.0217 & 1.0000 & \\
  \multicolumn{1}{l}{$\overline{S}$} & 0.7946 & 0.0355 & 0.1195 & 0.1192 & 0.2499 & 66\\
  \multicolumn{1}{l}{$\widehat{S}$} & 0.6533 & 0.0546 & 0.0602 & 0.0611 & 0.2451 & \\\hline

  \multicolumn{1}{l}{$S$} & 0.6965 & 0.0158 & 0 & 0.0158 & 1.0000 & \\
  \multicolumn{1}{l}{$\overline{S}$} & 0.7772 & 0.0312 & 0.0860 & 0.0866 & 0.3596 & 100\\
  \multicolumn{1}{l}{$\widehat{S}$} & 0.6738 & 0.0454 & 0.0483 & 0.0507 & 0.3422 & \\\hline

  \multicolumn{1}{l}{$S$} & 0.7141 & 0.0090 & 0 & 0.0090 &1.0000 & \\
  \multicolumn{1}{l}{$\overline{S}$} & 0.7573 & 0.0228 & 0.0487 & 0.0489 & 0.2277 & 200\\
  \multicolumn{1}{l}{$\widehat{S}$} & 0.6991 & 0.0298 & 0.0327 & 0.0334 & 0.2288 & \\
  \bottomrule
\end{tabular}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

